LocationSafe: Granular Location Privacy for IoT Devices

Today, mobile data owners lack consent and control over the release and utilization of their location data. Third party applications continuously process and access location data without data owners granular control and without knowledge of how location data is being used. The proliferation of IoT devices will lead to larger scale abuses of trust. In this paper we present the first design and implementation of a privacy module built into the GPSD daemon. The GPSD daemon is a low-level GPS interface that runs on GPS enabled devices. The integration of the privacy module ensures that data owners have granular control over the release of their GPS location. We describe the design of our privacy module and then evaluate the performance of private GPS release and demonstrate that strong privacy guarantees can be built into the GPSD daemon itself with minimal to no overhead.

==> background.tex <==
\section{Background}

\subsection{GPSD}

user side GPS daemon for linux/android system
interacts with swappable GPS drivers and kernel to read raw GPS
            data
            
            has lock on GPS device so all apps have to go through daemon for
            GPS Ddata. apps are not able to directly access the GPS sensor.
            
provides GPS data in form of JSON through a port

\subsection{Privacy Module}

        User specifies 2 things
        ACCURACY(geographical range)
        RATE(how often data sent)
